Distributed MST: A Smoothed Analysis

We study smoothed analysis of distributed graph algorithms, focusing on the fundamental minimum spanning tree (MST) problem. With the goal of studying the time complexity of distributed MST as a function of the "perturbation" of the input graph, we posit a {\em smoothing model} that is parameterized by a smoothing parameter $0 \leq \epsilon(n) \leq 1$ which controls the amount of {\em random} edges that can be added to an input graph $G$ per round. Informally, $\epsilon(n)$ is the probability (typically a small function of $n$, e.g., $n^{-\frac{1}{4}}$) that a random edge can be added to a node per round. The added random edges, once they are added, can be used (only) for communication. We show upper and lower bounds on the time complexity of distributed MST in the above smoothing model. We present a distributed algorithm that, with high probability,\footnote{Throughout, with high probability (whp) means with probability at least $1 - n^{-c}$, for some fixed, positive constant $c$.} computes an MST and runs in $\tilde{O}(\min\{\frac{1}{\sqrt{\epsilon(n)}} 2^{O(\sqrt{\log n})}, D + \sqrt{n}\})$ rounds\footnote{The notation $\tilde{O}$ hides a $\polylog(n)$ factor and $\tilde{\Omega}$ hides a $\frac{1}{\polylog{(n)}}$ factor, where $n$ is the number of nodes of the graph.} where $\epsilon$ is the smoothing parameter, $D$ is the network diameter and $n$ is the network size. To complement our upper bound, we also show a lower bound of $\tilde{\Omega}(\min\{\frac{1}{\sqrt{\epsilon(n)}}, D+\sqrt{n}\})$. We note that the upper and lower bounds essentially match except for a multiplicative $2^{O(\sqrt{\log n})} \polylog(n)$ factor. Our work can be considered as a first step in understanding the smoothed complexity of distributed graph algorithms.

==> other_smoothing_models_algorithm_for_M_k_star.tex <==
\subsection{An MST algorithm for $\mathcal{M}(k, *)$ with $k  =  \tilde{\Theta}(n^{\frac{3}{4}})$} \label{section-algorithm-for-alternative-smoothing-model}





We give a rough sketch of an algorithm that computes an MST in this smoothing model in $O(n^{\frac{1}{4}}) \cdot 2^{O(\sqrt{\log{n}})}$ time (rounds). Let $G(V,E)$ be the original graph, and $S$ be the set of added smoothed edges.



\begin{enumerate}


    \item Run \emph{controlled GHS} \cite{Garay_1998} for $\frac{\log{n}}{4}$ phases. This takes $\tilde{O}(n^{\frac{1}{4}})$ rounds. Every cluster (each of which is locally an MST now) will now have diameter $O(n^{\frac{1}{4}})$, and there will be $O(n^{\frac{3}{4}})$ such clusters \cite[Corollary 3.5]{Garay_1998}.

    
    \item View these clusters as a set of \emph{super-nodes}, denoted $V'$. Let $E' \subset E$ be the set of inter-super-node edges, let $S' \subset S$ be the set of inter-super-node smoothed edges. Consider two super-graphs: $G'(V',E')$ and $R'(V',S')$. It is easy to show that due to the $k  =  \tilde{O}(n^{\frac{3}{4}})$ random edges introduced by the \emph{smoothing} process, the super-graph $R'(V',S')$  is essentially an Erdős–Rényi random graph or a $R'(n', p)$-random graph, where
    \begin{equation}
        n' = O(n^{\frac{3}{4}})
    \end{equation}
    and
    \begin{equation}
        p = \Omega(\frac{\ln{(n')}}{n'})
    \end{equation}
    Essentially, the super-graphs $G' \cup R'$ is equivalent to the smoothed graph of our model in Section \ref{sec:model}.
        
    % \soumyottam{Note that $n'$ may even be smaller than $\Theta(n^{\frac{3}{4}})$, but that's not a problem for us. That's actually even better, informally speaking. Because, with a smaller value of $n'$, the number of smoothed edges $k$ becomes larger in comparison. That is, the resultant (super-)graph becomes even ``denser'' compared to the $G(n', p)$-random graph described above.}

    \item Solve the MST problem for the super-graph $G'$, using the routing structure by Ghaffari et al.\ \cite{Ghaffari_2017_PODC, Ghaffari_2018_DISC}, and our MST algorithm with $k$-aggregate routing, which perform routing over $R'$. To implement the algorithm on the super-graph, we simply pipeline messages within all the super-nodes. This step takes $O(\log{n})$ phases. where each phase takes
    \begin{center}
        $O(n^{\frac{1}{4}}) \cdot 2^{O(\sqrt{\log n})}$ rounds,
    \end{center}    
    The extra term of $O(n^{\frac{1}{4}})$ is incurred by the inner super-node pipelining. 

    Thus, in total, this step takes $O(n^{\frac{1}{4}} \cdot \log{n}) \cdot 2^{O(\sqrt{\log n})}$ rounds.

    
    \item Combining the MST over the super-graph $G'$, and the MSTs in each super-node, we have the MST for the original graph. Therefore, the total time complexity of the algorithm is
    \begin{align}
        &O(n^{\frac{1}{4}})  +  O(n^{\frac{1}{4}} \cdot \log{n}) \cdot 2^{O(\sqrt{\log n})}   \nonumber \\
        &=   O(n^{\frac{1}{4}}) \cdot 2^{O(\sqrt{\log n})}
    \end{align}
    
    
\end{enumerate}
% We note that this is equivalent to the same bounds
%     obtained for the $\epsilon$-smoothing model
%     for a suitably chosen $\epsilon$, i.e., $\epsilon  = k/n$. 
% \pham{This is multiplicative, so not equivalent to the addictive bound.}

\subsection{Approaching the lower bound}
We can improve the analysis with the $\mathcal{M}(k, *)$ model, choosing 
$k=\Theta(n\sqrt{\epsilon} \log{n})$, where $\epsilon = \poly(n)$. Let $G(V,E)$ be the original graph, and $S$ be the set of added smoothed edges.

\begin{enumerate}
    \item Run \emph{controlled GHS} \cite{Garay_1998} for $\\log{\frac{1}{\sqrt{\epsilon}}}$ phases. This takes $O(\frac{\log{n}}{\sqrt{\epsilon}})$ rounds. Every cluster (each of which is locally an MST now) will now have diameter $O(\frac{1}{\sqrt{\epsilon}})$, and there will be $O(n\sqrt{\epsilon})$ such clusters \cite[Corollary 3.5]{Garay_1998}.

    
    \item View these clusters as a set of \emph{super-nodes}, denoted $V'$. Let $E' \subset E$ be the set of inter-super-node edges, let $S' \subset S$ be the set of inter-super-node smoothed edges. Consider two super-graphs: $G'(V',E')$ and $R'(V',S')$. It is easy to show that due to the $k  =  \Theta(n\sqrt{\epsilon} \log{n})$ random edges introduced by the \emph{smoothing} process, with the condition $\epsilon = \poly(n)$, the super-graph $R'(V',S')$  is essentially an Erdős–Rényi random graph or a $R'(n', p)$-random graph, where
    \begin{equation}
        n' = O(n \sqrt{\epsilon})
    \end{equation}
    and
    \begin{equation}
        p = \Omega(\frac{\ln{(n')}}{n'})
    \end{equation}
    Essentially, the super-graphs $G' \cup R'$ is equivalent to the smoothed graph of our model in Section \ref{sec:model}.

    \item Solve the MST problem for the super-graph $G'$, using the routing structure by Ghaffari et al.\ \cite{Ghaffari_2017_PODC, Ghaffari_2018_DISC}, and our MST algorithm with $k$-aggregate routing, which perform routing over $R'$. To implement the algorithm on the super-graph, we simply pipeline messages within all the super-nodes. This step takes $O(\log{n})$ phases. where each phase takes
    \begin{center}
        $O(\frac{1}{\sqrt{\epsilon}}) \cdot 2^{O(\sqrt{\log n})}$ rounds,
    \end{center}    
    The extra term of $O(\frac{1}{\sqrt{\epsilon}})$ is incurred by the inner super-node pipelining. 

    Thus, in total, this step takes $O(\frac{1}{\sqrt{\epsilon}} \cdot \log{n}) \cdot 2^{O(\sqrt{\log n})}$ rounds.

    
    \item Combining the MST over the super-graph $G'$, and the MSTs in each super-node, we have the MST for the original graph. Therefore, the total time complexity of the algorithm is
    \begin{align}
        &O(\frac{\log{n}}{\sqrt{\epsilon}})  +  O(\frac{\log{n}}{\sqrt{\epsilon}}) \cdot 2^{O(\sqrt{\log n})}   \nonumber \\
        &=   O(\frac{\log{n}}{\sqrt{\epsilon}}) \cdot 2^{O(\sqrt{\log n})}
    \end{align}
    
\end{enumerate}

\subsubsection{Convert to the $\epsilon$-smoothing model}
We give a weak conversion of the $\mathcal{M}(k, *)$ to the original smoothing model with a suitable $\epsilon$. We consider these conditions: $k$ is small enough, such that $\epsilon = o(n)$, and the algorithm spend smoothing rounds to add smoothed edges before using them.

We approximate the probability of a smooth edges. In the $\mathcal{M}(k, *)$ model, $p = \frac{k}{n^2}$. In the $\epsilon$-smoothing model, after $l$ steps:
\begin{equation}
    p' = 1 - \left( 1 - \frac{\epsilon}{n} \right)^{2l}
    \approx \frac{2l\epsilon}{n}
\end{equation}
Thus $l\epsilon = \frac{k}{2n}$. The algorithm that approach the lower bound in $\mathcal{M}(k=n\epsilon'\log{n}, *)$, is equivalent to the same algorithm in $\epsilon$-smoothing model, with $\epsilon = \epsilon'$, and $l = \frac{\log{n}}{2\sqrt{\epsilon}}$ rounds of smoothing, and hence the running time is the same.
